Fixed and Market Pricing for Cloud Services

We study a model of congestible resources, where pricing and scheduling are intertwined. Motivated by the problem of pricing cloud instances, we model a cloud computing service as linked $GI/GI/\cdot$ queuing systems where the provider chooses to offer a fixed pricing service, a dynamic market based service, or a hybrid of both, where jobs can be preempted in the market-based service. Users (jobs), who are heterogeneous in both the value they place on service and their cost for waiting, then choose between the services offered. Combining insights from auction theory with queuing theory we are able to characterize user equilibrium behavior, and show its insensitivity to the precise market design mechanism used. We then provide theoretical and simulation based evidence suggesting that a fixed price typically, though not always, generates a higher expected revenue than the hybrid system for the provider.

==> My-defn-shorthands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My standard definitions and shorthands %

%% Environment definitions
%\theoremstyle{plain} \newtheorem{lemma}{Lemma}
%\theoremstyle{plain} \newtheorem{proposition}{Proposition}
%\theoremstyle{plain} \newtheorem{theorem}{Theorem}
%\theoremstyle{definition} \newtheorem{corollary}{Corollary}
%\theoremstyle{definition} \newtheorem{definition}{Definition}
%\theoremstyle{definition} \newtheorem{assumption}{Assumption}
%\theoremstyle{definition} \newtheorem{example}{Example}
%
%% Environment definitions without numbering
%\theoremstyle{plain} \newtheorem*{lemma*}{Lemma}
%\theoremstyle{plain} \newtheorem*{proposition*}{Proposition}
%\theoremstyle{plain} \newtheorem*{theorem*}{Theorem}
%\theoremstyle{definition} \newtheorem*{corollary*}{Corollary}
%\theoremstyle{definition} \newtheorem*{definition*}{Definition}
%\theoremstyle{definition} \newtheorem*{assumption*}{Assumption}
%\theoremstyle{definition} \newtheorem*{example*}{Example}

% Standard sets
\newcommand{\R}{\ensuremath{\mathbb{R}}}										% Real numbers
\newcommand{\N}{\ensuremath{\mathbb{R}}}										% Natural numbers
\newcommand{\Z}{\ensuremath{\mathbb{R}}}										% Integers
 
% Maximum and minimum, argmax etc
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\maximize}{\operatornamewithlimits{maximize}}
\newcommand{\minimize}{\operatornamewithlimits{minimize}}

% Operators
\newcommand{\E}[1]{\mathbb{E}\left[#1\right]}								% Expectation
\newcommand{\Ebig}[1]{\mathbb{E}\big[#1\big]}
\newcommand{\Ebigg}[1]{\mathbb{E}\bigg[#1\bigg]}
\newcommand{\CE}[2]{\mathbb{E}\left[#1 \left\vert\right. #2 \right]}	% Conditional Expectation
\newcommand{\Prob}[1]{\mathbb{P}\left[#1\right]}						% Probability
\newcommand{\CProb}[2]{\mathbb{P}\left[#1 \left\vert\right. #2 \right]}	% Conditional probability
\newcommand{\pos}[1]{\left[#1\right]^{+}}										% Positive function
\newcommand{\posbig}[1]{\big[#1\big]^{+}}
\newcommand{\posbigg}[1]{\bigg[#1\bigg]^{+}}
\newcommand{\indicator}[1]{\textbf{1}_{\left\{#1\right\}}} 	% Indicator function
\newcommand{\od}[2]{\frac{d #1}{d #2}}											% Oridnary derivative
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}				% Partial derivative

% Shorthands
\newcommand{\mb}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\bs}[1]{\boldsymbol #1}													% For bold greek letters for which \mathbf doesn't work
\newcommand{\mc}[1]{\ensuremath{\mathcal{#1}}}							% Shorthand for matcal
\newcommand{\wh}[1]{\widehat{#1}}														% Shorthand for \widehat
\newcommand{\wt}[1]{\widetilde{#1}}													% Shorthand for \widetilde

\newcommand{\beq}[1]{\begin{equation} \label{eq:#1}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqn}{\begin{equation*}}
\newcommand{\eeqn}{\end{equation*}}
\newcommand{\eref}[1]{\eqref{eq:#1}}

%\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]} 
% Controls the number with \thanks in case of multiple authors. \samethanks[0] will put no number. 
% If say author 1 and 2 have the same affiliation, then use \thanks and then \samethanks or \samethanks[1]. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Documents specific definitions
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> My-packages.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My standard set of packages %
		% To use the command \sfrac{}{} for slanted inline fraction
\usepackage{times}			% Changes the font to save space

% \usepackage[comma]{natbib}		  % Allows use of different types of citations

% For pdf bookmarks and hyperlinks. This needs to be the last package in the document. 
% Check documentation. linkbordercolor={R G B}
% \usepackage[bookmarks=true, linkbordercolor={1 1 1}, citebordercolor={1 1 1}]{hyperref}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
